To be Robust or to be Fair: Towards Fairness in Adversarial Training

Adversarial training algorithms have been proved to be reliable to improve machine learning models' robustness against adversarial examples. However, we find that adversarial training algorithms tend to introduce severe disparity of accuracy and robustness between different groups of data. For instance, a PGD adversarially trained ResNet18 model on CIFAR-10 has 93% clean accuracy and 67% PGD l-infty-8 robust accuracy on the class "automobile" but only 65% and 17% on the class "cat". This phenomenon happens in balanced datasets and does not exist in naturally trained models when only using clean samples. In this work, we empirically and theoretically show that this phenomenon can happen under general adversarial training algorithms which minimize DNN models' robust errors. Motivated by these findings, we propose a Fair-Robust-Learning (FRL) framework to mitigate this unfairness problem when doing adversarial defenses. Experimental results validate the effectiveness of FRL.

==> sections/unused_tables.tex <==



\begin{table*}[t]
\centering
\caption{Different adversarial training algorithms under $l_\infty$-norm 8/255 adversarial perturbation budget on CIFAR10 dataset (PreAct ResNet18 (above) and Wide ResNet28(below)). We report the average standard error and robust error (evaluated under PGD attack by $8/255$), as well as the worst / best standard error and robust error among all classes.} 
\scalebox{0.8}{
\begin{tabular}{c |c c c | c c c} 
\hline
& \textbf{Avg. Std.} & \textbf{Best Std.} & \textbf{Worst Std.} & \textbf{Avg. Robust} & \textbf{Best Robust} & \textbf{Worst Robust}  \\  
\hline\hline
\textbf{Natural Training} & 5.1 &  1.8  & 11.3  & 0.0  & 0.0 & 0.0 \\
\textbf{PGD Adv. Training} & 15.5 &  6.1  & 33.8  & 56.4  & 34.3 & 85.7 \\
\textbf{PGD Adv. Train + Early Stop} & 16.8 & 4.8  & 41.7  & 49.3  & 31.6 & 79.0 \\
%\textbf{TRADES $(\beta = 1)$} & 85.6 & 42.0  & 72.1  &  95.3  & 16.4 & 68.1\\
\textbf{TRADES ($1/\lambda = 1$)} & 14.6 & 5.0 & 31.2 & 57.7 & 31.0 & 84.7 \\
\textbf{TRADES ($1/\lambda = 6$)} & 19.6 & 6.5 & 39.1 & 49.4 & 24.3 & 77.6 \\\
\textbf{MART} & ? & ? & ? & ? & ? & ? \\
\hline\hline
\textbf{Natural Training} & 4.8 & 1.7  & 10.5  & 0.0  & 0.0 & 0.0 \\
\textbf{PGD Adv. Training} & 13.6 & 6.2  & 30.5  & 52.8  & 31.7 & 81.4 \\
\textbf{PGD Adv. Train + Early Stop} & 14.1 & 4.5  & 27.9  & 48.6  & 25.6 & 74.7 \\
%\textbf{TRADES $(\beta = 1)$} & 85.6 & 42.0  & 72.1  &  95.3  & 16.4 & 68.1\\
\textbf{TRADES ($1/\lambda = 1$)} & 12.6 & 4.2 & 22.4 & 52.8 & 28.1 & 76.7 \\
\textbf{TRADES ($1/\lambda = 6$)} & 16.2 & 5.5 & 28.5 & 47.2 & 23.2 & 71.8 \\
\textbf{MART} & ? & ? & ? & ? & ? & ? \\
\hline
\end{tabular}}
\label{tab:fact2}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!]
\centering
\caption{Different adversarial training algorithms under $l_2$-norm 0.5 adversarial perturbation budget on CIFAR10 dataset (PreAct ResNet18 (above) and Wide ResNet28(below)). We report the average standard error and robust error (evaluated under PGD attack by $0.5$), as well as the worst / best standard error and robust error among all classes.} %Note that $\beta$ controls the TRADES's accuracy-robustness trade-off. Large $\beta$ gives higher stress on robustness.}
\scalebox{0.8}{
\begin{tabular}{c |c c c | c c c} 
\hline
& \textbf{Avg. Std.} & \textbf{Best Std.} & \textbf{Worst Std.} & \textbf{Avg. Robust} & \textbf{Best Robust} & \textbf{Worst Robust}  \\  
\hline\hline
\textbf{Natural Training} & 5.1 &  1.8  & 11.3  & 0.0  & 0.0 & 0.0 \\
\textbf{PGD Adv. Training} & 15.5 &  6.1  & 33.8  & 56.4  & 34.3 & 85.7 \\
\textbf{PGD Adv. Train + Early Stop} & 16.8 & 4.8  & 41.7  & 49.3  & 31.6 & 79.0 \\
%\textbf{TRADES $(\beta = 1)$} & 85.6 & 42.0  & 72.1  &  95.3  & 16.4 & 68.1\\
\textbf{TRADES ($1/\lambda = 1$)} & 14.6 & 5.0 & 31.2 & 57.7 & 31.0 & 84.7 \\
\textbf{TRADES ($1/\lambda = 6$)} & 19.6 & 6.5 & 39.1 & 49.4 & 24.3 & 77.6 \\\
\textbf{MART} & ? & ? & ? & ? & ? & ? \\
\hline\hline
\textbf{Natural Training} & 4.8 & 1.7  & 10.5  & 0.0  & 0.0 & 0.0 \\
\textbf{PGD Adv. Training} & 13.6 & 6.2  & 30.5  & 52.8  & 31.7 & 81.4 \\
\textbf{PGD Adv. Train + Early Stop} & 14.1 & 4.5  & 27.9  & 48.6  & 25.6 & 74.7 \\
%\textbf{TRADES $(\beta = 1)$} & 85.6 & 42.0  & 72.1  &  95.3  & 16.4 & 68.1\\
\textbf{TRADES ($1/\lambda = 1$)} & 12.6 & 4.2 & 22.4 & 52.8 & 28.1 & 76.7 \\
\textbf{TRADES ($1/\lambda = 6$)} & 16.2 & 5.5 & 28.5 & 47.2 & 23.2 & 71.8 \\
\textbf{MART} & ? & ? & ? & ? & ? & ? \\
\hline
\end{tabular}}
\label{tab:fact3}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!]
\centering
\caption{For adversarial defenses algorithms towards $l_2$-norm 0.5 adversarial perturbation budget on CIFAR10 dataset. We also report the fairness conditions of certified defenses methods, such as randomized smoothing.} %Note that $\beta$ controls the TRADES's accuracy-robustness trade-off. Large $\beta$ gives higher stress on robustness.}
\scalebox{0.8}{
\begin{tabular}{c |c c c | c c c} 
\hline
& \textbf{Avg. Std.} & \textbf{Best Std.} & \textbf{Worst Std.} & \textbf{Avg. Robust} & \textbf{Best Robust} & \textbf{Worst Robust}  \\  
\hline\hline
\textbf{Natural Training} & 5.1 &  1.8  & 11.3  & 0.0  & 0.0 & 0.0 \\
\textbf{PGD Adv. Training} & 15.5 &  6.1  & 33.8  & 56.4  & 34.3 & 85.7 \\
\textbf{PGD Adv. Train + Early Stop} & 16.8 & 4.8  & 41.7  & 49.3  & 31.6 & 79.0 \\
\hline
\end{tabular}}
\label{tab:fact4}
\end{table*}



\subsection{Robust / Non-Robust Features}
In this section, we discuss the robust fairness issues in the setting which is motivated by the work~\cite{tsipras2018robustness, ilyas2019adversarial}, which specifically split the data features into two categories: robust features and non-robust features. Formally, the data distribution are as following:
\begin{spreadlines}{0.8em}
\begin{align}
\small
\label{eq:data_dist2}
\begin{split}
    & y \stackrel{u.a.r}{\sim} \{-1, +1\},~~~ \theta = ( \overbrace{\eta,...,\eta}^\text{dim = d}, \overbrace{\gamma,...,\gamma}^\text{dim = m}),~~~
    \\ &x \sim  
    \begin{cases}
      ~~\mathcal{N}~(\theta, \sigma_{+1}^2I) ~~~~&\text{if $y= + 1$}\\
      ~~\mathcal{N}~(-\theta, \sigma_{-1}^2I) ~~~~&\text{if $y= - 1$}\\
    \end{cases} 
\end{split}
\end{align}
\end{spreadlines}
where in the center vector $\theta$, it includes robust features with scale $\eta > \epsilon$, and non-robust features with scale $\gamma < \epsilon$. Typically non-robust feature space has much higher dimension than robust feature space ($m>>d$).
The main story of the works~\cite{tsipras2018robustness, ilyas2019adversarial} is that: natural models' prediction depends on the high-dimensional non-robust features; robust models' prediction depends on the low-dimensional robust features. Because robust models use much fewer features to do classification, they will have larger standard errors but less suffer from attacks.


In our work, we show that if there is a $K$-factor difference between two classes variance: $\sigma_{+1}:\sigma_{-1}= K$, there will be a strong error disparity. Note that we use $Z_\text{nat}(f;\pm 1)$ to denote the Z-score of corresponding error rates $\mathcal{R}_\text{nat}(f;\pm 1)$~\footnotemark[3]. We have the following results:
\begin{align}
\label{eq:zscores}
\begin{split}
    &\begin{cases}
     Z_\text{nat}(f_\text{nat};-1) &= c\cdot A - K\sqrt{c^2 \cdot A^2 + q(K)} \\
    Z_\text{nat}(f_\text{nat};+1) &= -K\cdot c\cdot A + \sqrt{c^2 \cdot A^2 + q(K)} \\
    \end{cases}\\
    &\begin{cases}
     Z_\text{nat}(f_\text{rob};-1) &= c\cdot B - K\sqrt{c^2 \cdot B^2 + q(K)} - \frac{\sqrt{d}}{\sigma}\epsilon  \\
    Z_\text{nat}(f_\text{rob};+1) &= -K\cdot c\cdot B + \sqrt{c^2 \cdot B^2 + q(K)} - \frac{\sqrt{d}}{K\sigma}\epsilon \\
    \end{cases}\\
\end{split}
\end{align}
where $c$ is constant, $q(K) = \frac{2logK}{K^2-1}$. Note that if $K=1$, then $q(K)=0$, so the two classes will have the same errors. The key elements in Eq.\ref{eq:zscores} are $A = \sqrt{d\eta^2 + m\gamma^2}$ and $B = \sqrt{d\eta^2}$. For example, consider the class ``-1'', since $K>1$ and $m>>d$, the robust model's Z-score $Z_\text{nat}(f_\text{nat};-1)$ grows approximately $\frac{B}{A}$ times after adversarial training (if we last term $\frac{\sqrt{d}}{\sigma}\epsilon$). Similarly, the Z-score of class ``+1'' will also grow $\frac{B}{A}$ times after adversarial training. Intuitively, imagine that the original error gap ($Z_\text{nat}(f_\text{nat};+1) - Z_\text{nat}(f_\text{nat};-1)$) in a natural model is small, but adversarial training ``scales up'' the errors for each class at the same rate $\frac{B}{A}$, the error gap in robust models ($Z_\text{nat}(f_\text{rob};+1) - Z_\text{nat}(f_\text{rob};-1)$) is also $\frac{B}{A}$ times larger. As a result, there is a much larger error different between classes ``$\pm 1$'' in robust models. The robust errors will also have similar results, which we put the detailed discussions in Appendix. As a conclusion, in Section~\ref{sec:deep_example}, we discuss the case that if adversarial training increases overall standard errors, it may also increase the errors for each class by  consistent rates. Thus, a robust model can present a stronger class-wise performance disparity.

